Drawing the LINE: Cryptographic Analysis and Security Improvements for the LINE E2EE Protocol

LINE has emerged as one of the most popular communication platforms in many East Asian countries, including Thailand and Japan, with millions of active users. Therefore, it is essential to understand its security guarantees. In this work, we present the first provable security analysis of the LINE version two (LINEv2) messaging protocol, focusing on its cryptographic guarantees in a real-world setting. We capture the architecture and security of the LINE messaging protocol by modifying the Multi-Stage Key Exchange (MSKE) model, a framework for analysing cryptographic protocols under adversarial conditions. While LINEv2 achieves basic security properties such as key indistinguishability and message authentication, we highlight the lack of forward secrecy (FS) and post-compromise security (PCS). To address this, we introduce a stronger version of the LINE protocol, introducing FS and PCS to LINE, analysing and benchmarking our results.

==> SM_security.tex <==
\fbox{
\begin{minipage}{0.22\textwidth}
\hspace{0.25cm}
    \underline{$\initO$}
    \begin{algorithmic}[1]
    \State $\key \getsr \KeySpace$
    \State $\state_A \gets \initA(\key)$ 
    \State $\state_A \gets \initA(\key)$ 
    \State $(\epoch_A,\epoch_B) \gets (0,0)$ 
    \State $\indexsm_A,\indexsm_B \gets 0$ 
    \State $\epoch_L \gets -\infty$ 
    \State $\trans, \chall, \comp \gets \emptyset$ 
    \State $b \tor \bits$  
    \end{algorithmic}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{0.25cm}
    \underline{$\corrA$}
    \begin{algorithmic}[1]
    \State $\req ~B \not\in \chall$
    \If {$\compS = true$}
    \State $\comp \getplus \trans(B)$
    \State $\epoch_L \gets max(\epoch_A, \epoch_B)$
    \EndIf
    \State \Return $\state_A$
    \end{algorithmic} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{0.25cm}
    \underline{$\transmitA(\msg,\random)$}
    \begin{algorithmic}[1]
    \State $(\random,\flag) \gets \SamIfNec(\random)$
    \State $\epmgmt (A,\flag)$
    \State $\indexsm_A++$
    \State $(\state_A,\ciphertxt) \gets \send(\state_A,\msg;\random)$
    \State $\record(A,norm,\msg,\ciphertxt)$
    \State \Return $\ciphertxt$
    \end{algorithmic} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{0.25cm}
    \underline{$\challA(\msg_0,\msg_1,\random)$}
    \begin{algorithmic}[1]
    \State $(\random,\flag) \gets \SamIfNec(\random)$ 
    \State $\epmgmt(A,\flag)$
    \State $\req \safech_A ~and |\msg_0| = |\msg_1|$ 
    \State $\indexsm_A ++$
    \State $(\state_A,\ciphertxt) \gets \send(\msg_b;\random)$
    \State $\record(A,\chall,\msg_b,\ciphertxt)$
    \State \Return $\ciphertxt$
    \end{algorithmic}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{0.25cm}
    \underline{$\deliverA(\ciphertxt)$}
    \begin{algorithmic}[1]
    \State$ \req (B,\epoch,\indexsm,\msg,\ciphertxt) \in \trans$
    \State $for ~some ~\epoch,\indexsm,\msg$
    \State $(\state_A,\epoch',\indexsm',\msg') \gets \Rcv(\state_A,\ciphertxt) $
    \If{$(\epoch',\indexsm',\msg') \neq (\epoch,\indexsm,\msg)$}
    \State $\win$
    \If{$(\epoch,\indexsm,\msg) \in \chall$}
    \State $\msg' \gets \bot$
    \EndIf
    \EndIf
    \State $\epoch_A \gets max(\epoch_A,\epoch_B)$
    \State $\delete(\epoch,\indexsm)$
    \State \Return $(\epoch',\indexsm',\msg')$
    \end{algorithmic}
    \end{minipage}
\vline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}{0.22\textwidth}
\hspace{0.25cm}
    \underline{$\injectA(\ciphertxt)$}
    \begin{algorithmic}[1]
    \State $\req ~ (B,\ciphertxt) \not\in \trans~and~\safeinj$
    \State $(\state_A,\epoch',\indexsm',\msg') \gets \Rcv(\state_A,\ciphertxt)$ 
    \If{$\msg' \neq \bot ~and ~(B,\epoch',\indexsm') \not\in \comp$}
    \State $\win$
    \EndIf
    \State $\epoch_A \gets max(\epoch_A,\epoch')$ 
    \State $\delete (\epoch',\indexsm')$
    \State \Return $(\epoch',\indexsm',\msg')$
    \end{algorithmic}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{0.25cm}
    \underline{$\epmgmt(P,\flag)$}
    \begin{algorithmic}[1]
    \If{$P = A ~and ~\epoch_P~even ~or P = B ~and \epoch_P ~odd$}
    \If {$\flag = bad ~and \urcorner \safech_P$}
    \State $\epoch_L \gets \epoch_P +1$
    \EndIf
    \EndIf
    \State $\epoch_P++$
    \State $\indexsm_P \gets 0$
    \end{algorithmic}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{0.25cm}
    \underline{$\SamIfNec(\random)$}
    \begin{algorithmic}[1]
    \State $\flag \gets bad$
    \If{$\random = \bot$}
    \State $\random \getsr \RandomSpace$
    \State $\flag \gets good$ 
    \EndIf
    \State \Return $(\random,\flag)$
    \end{algorithmic}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{0.25cm}
    \underline{$\record(P,\flag,\msg,\ciphertxt)$}
    \begin{algorithmic}[1]
    \State $\rec \gets (P,\epoch_P,\indexsm_P,\msg,\ciphertxt)$
    \State $\trans \getplus \rec$
    \If{$\urcorner \safech_P$}
    \State $\comp \getplus \rec$
    \EndIf
    \If{$\flag = \chall$}
    \State $\chall \getplus \rec$  
    \EndIf
    \end{algorithmic}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{0.25cm}
\underline{$\delete(\epoch,\indexsm)$}
    \begin{algorithmic}[1]
    \State $\rec \gets (P,\epoch,\indexsm_P,\msg,\ciphertxt)$ 
    \State $for ~some ~P,\msg,\ciphertxt$ 
    \State $\trans,\chall,\comp \getminus \rec$
    \State $\safech_P :\Longleftrightarrow \epoch_p \geq \epoch_L + \Delta_{\SM}$
    \State $\safeinj :\Longleftrightarrow min(\epoch_A,\epoch_B) \geq \epoch_L +$ 
    \State $\Delta_{\SM}$
    \end{algorithmic}
   \vspace{0.5cm}
 \end{minipage}
}


==> crypto-macros.tex <==
% always check cryptocode First

\tikzstyle{player} = [rectangle, minimum width=2cm, minimum height=1cm, text centered, draw=black, fill=mLightBrown!50]
\tikzstyle{adversary} = [rectangle, minimum width=2cm, minimum height=1cm, text centered, draw=black, fill=red!50]
% TEXT COMMANDS
%\newcommand{\etal}{et~al.\xspace{}}
%\newcommand{\ie}{i.e.~}
%\newcommand{\eg}{e.g.~}
%\newcommand{\ppttxt}{probabilistic polynomial-time}
%\mathchardef\mhyphen="2D

%% FIGURE COMMANDS
\definecolor{mBlue}{HTML}{22a1dc}
\definecolor{sBlue}{HTML}{009FE3}
\definecolor{sYellow}{HTML}{FFED00}
\definecolor{sRed}{HTML}{E30613}
\definecolor{sGreen}{HTML}{009640}
\definecolor{sPurple}{HTML}{440099}
\definecolor{sOrange}{HTML}{EB641E}
\definecolor{mGreen}{HTML}{86cd30}
\definecolor{darkgreen}{HTML}{006400}
\definecolor{mLightBrown}{HTML}{e68a00}
\definecolor{lightred}{HTML}{FF9999}

% COLOUR COMMANDS
\newcommand{\sBlue}[1]{\textcolor{sBlue}{#1}}
\newcommand{\sB}[1]{\sBlue{#1}}
\newcommand{\sRed}[1]{\textcolor{sRed}{#1}}
\newcommand{\sR}[1]{\sRed{#1}}
\newcommand{\sGreen}[1]{\textcolor{sGreen}{#1}}
\newcommand{\sG}[1]{\sGreen{#1}}
\newcommand{\sPurple}[1]{\textcolor{Purple}{#1}}
\newcommand{\sP}[1]{\sPurple{#1}}
\newcommand{\sYellow}[1]{\textcolor{sYellow}{#1}}
\newcommand{\sY}[1]{\sYellow{#1}}
\newcommand{\sOrange}[1]{\textcolor{sOrange}{#1}}
\newcommand{\sO}[1]{\sOrange{#1}}

\begin{comment}
    % STYLES
\newcommand{\styleAdversary}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\styleAlgorithm}[1]{\textsf{\upshape #1}}
\newcommand{\styleScheme}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\styleSecurityNotion}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\styleQueries}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\styleVariables}[1]{\ensuremath{\mathit{#1}}}
\newcommand{\styleConstants}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\styleProtocols}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\styleOracles}[1]{\ensuremath{\mathrm{#1}}}
\renewcommand{\O}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\V}[1]{\ensuremath{\mathit{#1}}}

%% FUNCTIONS, SAMPLERS, ETC
\newcommand{\getsr}{\ensuremath{\overset{\$}{\leftarrow}}}
\newcommand{\tor}{\ensuremath{\overset{\$}{\rightarrow}}}
\newcommand{\randcoin}[1]{\ensuremath{\mathcal{R}_{#1}}}
\newcommand{\maxover}[2]{\ensuremath{\underset{#1}{\mathsf{max}}\{#2\}}}
\newcommand{\bits}{\ensuremath{\{0,1\}}}
\newcommand{\rreplace}[1]{\ensuremath{\widetilde{#1}}}

%% GROUPS AND SPACES
\newcommand{\group}{\ensuremath{\mathbb{G}}}
\newcommand{\KeySpace}{\ensuremath{\mathcal{K}}}
\newcommand{\OutputSpace}{\ensuremath{\mathcal{O}}}
\newcommand{\InputSpace}{\ensuremath{\mathcal{I}}}
\newcommand{\NonceSpace}{\ensuremath{\mathcal{N}}}
\newcommand{\MessageSpace}{\ensuremath{\mathcal{M}}}
\newcommand{\HeaderSpace}{\ensuremath{\mathcal{H}}}
\newcommand{\RandomSpace}{\ensuremath{\mathcal{r}}}
\newcommand{\SaltSpace}{\ensuremath{\mathcal{S}}}

%% MATRIX STUFF
\newcommand{\matrixA}{\ensuremath
\end{comment}

{\mathbf{A}}}
\newcommand{\vectorU}{\ensuremath{\vec{u}}}

 %%DIFFIE-HELLMAN NOTATION
\renewcommand{\secpar}{\ensuremath{\lambda}}
\newcommand{\secparshort}{\ensuremath{k}}
\newcommand{\groupgen}{\ensuremath{\mathcal{G}}}
\newcommand{\generator}{\ensuremath{\V{g}}}

%% ALGORITHMS
\renewcommand{\adversary}{\ensuremath{\mathcal{A}}}
\newcommand{\state}{\ensuremath{st}}
\newcommand{\bdversary}{\ensuremath{\mathcal{B}}}
%\newcommand{\bdv}{\ensuremath{\mathcal{B}}}
\newcommand{\challenger}{\ensuremath{\mathcal{C}}}

%% PROTOCOLS AND ALGORITHMS
\newcommand{\KE}{\ensuremath{\mathsf{KE}}}
\newcommand{\ACCE}{\ensuremath{\mathsf{ACCE}}}
\newcommand{\AKeyGen}{\ensuremath{\mathsf{AKeyGen}}}
\newcommand{\ASKeyGen}{\ensuremath{\mathsf{ASKeyGen}}}
\newcommand{\SKeyGen}{\ensuremath{\mathsf{SKeyGen}}}
\newcommand{\PSKeyGen}{\ensuremath{\mathsf{PSKeyGen}}}
\newcommand{\EKeyGen}{\ensuremath{\mathsf{EKeyGen}}}
\newcommand{\EPKeyGen}{\ensuremath{\mathsf{EPKeyGen}}}
\newcommand{\KeyGen}{\ensuremath{\mathsf{KeyGen}}}
\newcommand{\Muck}{\ensuremath{\mathsf{Muckle}}}

% CRYPTO PRIMITIVES
\newcommand{\DHGen}{\ensuremath{\mathsf{DHGen}}}
\renewcommand{\DH}{\ensuremath{\mathsf{DH}}}
\newcommand{\Hash}{\ensuremath{\mathsf{H}}}
\newcommand{\AEAD}{\ensuremath{\mathsf{AEAD}}}
\newcommand{\Enc}{\ensuremath{\mathsf{Enc}}}
\newcommand{\Dec}{\ensuremath{\mathsf{Dec}}}
\newcommand{\dec}{\ensuremath{\mathsf{Dec}}}
\newcommand{\KDF}{\ensuremath{\mathsf{KDF}}}
\newcommand{\MAC}{\ensuremath{\mathsf{MAC}}}
\newcommand{\Timestamp}{\ensuremath{\mathsf{Timestamp}}}
\newcommand{\PRF}{\ensuremath{\mathsf{PRF}}}
\newcommand{\HKDF}{\ensuremath{\mathsf{HKDF}}}
\newcommand{\KEM}{\ensuremath{\mathsf{KEM}}}
\newcommand{\SIG}{\ensuremath{\mathsf{SIG}}}
\newcommand{\Expand}{\ensuremath{\mathsf{Exp}}}
\newcommand{\Extract}{\ensuremath{\mathsf{Ext}}}
% EXPERIMENT REGISTERS
\newcommand{\Adv}[2]{\ensuremath{\mathsf{Adv}^{#1}_{#2}}}
\newcommand{\Exp}[2]{\ensuremath{\mathsf{Exp}^{#1}_{#2}}}
\newcommand{\protocol}{\ensuremath{\Pi}}
\newcommand{\Dist}{\ensuremath{\mathcal{D}}}
\newcommand{\Prob}{\ensuremath{\mathsf{Pr}}}
\newcommand{\ctr}{\ensuremath{ctr}}
\newcommand{\vecPSK}[1]{\ensuremath{\vec{\mathsf{PSK}_{#1}}}}

% EXPERIMENT PREDICATES
\newcommand{\cleanpredicate}{\ensuremath{\mathsf{clean}}}

% EXPERIMENT CONSTANTS
\newcommand{\numParties}{\ensuremath{n_P}}
\newcommand{\numSessions}{\ensuremath{n_S}}
\newcommand{\numStages}{\ensuremath{n_T}}
\newcommand{\init}{\ensuremath{\styleConstants{init}}}
\newcommand{\resp}{\ensuremath{\styleConstants{resp}}}
\newcommand{\revealflag}{\ensuremath{\styleConstants{revealed}}}
\newcommand{\corruptflag}{\ensuremath{\styleConstants{corrupt}}}
\newcommand{\cleanflag}{\ensuremath{\styleConstants{clean}}}
\newcommand{\inprogress}{\ensuremath{\styleConstants{active}}}
\newcommand{\rejected}{\ensuremath{\styleConstants{reject}}}
\newcommand{\accepted}{\ensuremath{\styleConstants{accept}}}
\newcommand{\trueflag}{\ensuremath{\styleConstants{true}}}
\newcommand{\falseflag}{\ensuremath{\styleConstants{false}}}
%\newcommand{\numX}{\ensuremath{n_X}}

% EXPERIMENT FLAGS
\newcommand{\PSKflag}[1]{\ensuremath{\vec{\mathsf{PSKflag}_{#1}}}}
\newcommand{\SKflag}[1]{\ensuremath{\mathsf{SKflag}_{#1}}}
\newcommand{\ASKflag}[1]{\ensuremath{\mathsf{ASKflag}_{#1}}}
\newcommand{\AKflag}[1]{\ensuremath{\vec{\mathsf{AKflag}_{#1}}}}
\newcommand{\EPKflag}[1]{\ensuremath{\vec{\mathsf{EPKflag}_{#1}}}}
\newcommand{\EKflag}[1]{\ensuremath{\vec{\mathsf{EKflag}_{#1}}}}
\newcommand{\RSKflag}[1]{\ensuremath{\vec{\mathsf{RSKflag}_{#1}}}}
\newcommand{\RKflag}[1]{\ensuremath{\vec{\mathsf{RKflag}_{#1}}}}
\newcommand{\testflag}{\ensuremath{\mathsf{tested}}}

% SESSIONS AND PER-SESSION VARIABLES
\newcommand{\session}{\ensuremath{\pi}}
\newcommand{\sessionid}{\ensuremath{sid}}
\newcommand{\testsess}{\ensuremath{\pi^s_i}}
\newcommand{\partnersess}{\ensuremath{\pi^t_j}}
\newcommand{\partsess}{\ensuremath{\pi^r_j}}
\newcommand{\pk}{\ensuremath{pk}}
\newcommand{\sk}{\ensuremath{sk}}
\newcommand{\psk}{\ensuremath{psk}}
\newcommand{\pskid}{\ensuremath{pskid}}
\newcommand{\status}{\ensuremath{\alpha}}
\newcommand{\pid}{\ensuremath{pid}}
\newcommand{\kid}{\ensuremath{kid}}
\newcommand{\id}{\ensuremath{id}}
\newcommand{\ephkey}{\ensuremath{ek}}
\newcommand{\epubkey}{\ensuremath{epk}}
\renewcommand{\state}{\ensuremath{st}}
\newcommand{\msgsent}{\ensuremath{m_s}}
\newcommand{\msgrecd}{\ensuremath{m_r}}
\newcommand{\role}{\ensuremath{\rho}}

% SECURITY GAME QUERIES
\newcommand{\Test}{\ensuremath{\mathsf{Test}}}
\newcommand{\Corrupt}{\ensuremath{\mathsf{Corrupt}}}
\newcommand{\CorruptASK}{\ensuremath{\mathsf{CorruptASK}}}
\newcommand{\CorruptPK}{\ensuremath{\mathsf{CorruptPK}}}
\newcommand{\CorruptPSK}{\ensuremath{\mathsf{CorruptPSK}}}
\newcommand{\CorruptSK}{\ensuremath{\mathsf{CorruptSK}}}
\newcommand{\CorruptEPK}{\ensuremath{\mathsf{CorruptEPK}}}
\newcommand{\CorruptEK}{\ensuremath{\mathsf{CorruptEK}}}
\newcommand{\RevealRandom}{\ensuremath{\mathsf{RevealRandom}}}
\newcommand{\Reveal}{\ensuremath{\mathsf{Reveal}}}
\newcommand{\Create}{\ensuremath{\mathsf{Create}}}
\newcommand{\CreatePSK}{\ensuremath{\mathsf{CreatePSK}}}
\newcommand{\Send}{\ensuremath{\mathsf{Send}}}
\newcommand{\CompromiseQK}{\ensuremath{\mathsf{CompromiseQK}}}
\newcommand{\CompromiseSK}{\ensuremath{\mathsf{CompromiseSK}}}
\newcommand{\CompromiseSS}{\ensuremath{\mathsf{CompromiseSS}}}



%% SECURITY GAME NOTIONS
\newcommand{\COLL}{\styleSecurityNotion{coll}}
\newcommand{\coll}{\styleSecurityNotion{coll}}
\newcommand{\ddh}{\styleSecurityNotion{ddh}}
\newcommand{\dualkdf}{\styleSecurityNotion{dual}\mhyphen \styleSecurityNotion{kdf}}
\newcommand{\dualprf}{\styleSecurityNotion{dual}\mhyphen \styleSecurityNotion{prf}}
\newcommand{\prf}{\styleSecurityNotion{prf}}
\newcommand{\aead}{\styleSecurityNotion{aead}}
\newcommand{\auth}{\styleSecurityNotion{auth}}
\newcommand{\kdf}{\styleSecurityNotion{kdf}}
\newcommand{\PRFODH}{\ensuremath{\mathsf{PRFODH}}}
\newcommand{\eCKPFS}{\ensuremath{\mathsf{eCK}\mhyphen \mathsf{PFS}}}
\newcommand{\eCKPFSPSK}{\ensuremath{\mathsf{eCK}\mhyphen \mathsf{PFS} \mhyphen \mathsf{PSK}}}
\newcommand{\symlrPRFODH}{\ensuremath{\mathsf{sym}\mhyphen\mathsf{lr}\mhyphen \PRFODH}}
\newcommand{\lrPRFODH}{\ensuremath{\mathsf{lr}\mhyphen \PRFODH}}
\newcommand{\snPRFODH}{\ensuremath{\mathsf{sn}\mhyphen \PRFODH}}
\newcommand{\dualsnPRFODH}{\ensuremath{\mathsf{d}\mhyphen\mathsf{sn}\mhyphen \PRFODH}}
\newcommand{\ssPRFODH}{\ensuremath{\mathsf{ss}\mhyphen \PRFODH}}
\newcommand{\mnPRFODH}{\ensuremath{\mathsf{mn}\mhyphen \PRFODH}}
\newcommand{\msPRFODH}{\ensuremath{\mathsf{ms}\mhyphen \PRFODH}}
\newcommand{\mmPRFODH}{\ensuremath{\mathsf{mm}\mhyphen \PRFODH}}
\newcommand{\symsnPRFODH}{\ensuremath{\mathsf{sym}\mhyphen\mathsf{sn}\mhyphen \PRFODH}}
\newcommand{\symssPRFODH}{\ensuremath{\mathsf{sym}\mhyphen\mathsf{ss}\mhyphen \PRFODH}}
\newcommand{\symmsPRFODH}{\ensuremath{\mathsf{sym}\mhyphen\mathsf{ms}\mhyphen \PRFODH}}
\newcommand{\symmmPRFODH}{\ensuremath{\mathsf{sym}\mhyphen\mathsf{mm}\mhyphen \PRFODH}}
\newcommand{\symmnPRFODH}{\ensuremath{\mathsf{sym}\mhyphen\mathsf{mn}\mhyphen \PRFODH}}
%\newcommand{\ODH}{\ensuremath{\mathsf{ODH}}}
\newcommand{\eufqcma}{\ensuremath{\mathsf{q}\mhyphen\mathsf{euf}\mhyphen\mathsf{cma}}}
\newcommand{\EUFCMA}{\ensuremath{\mathsf{EUF}\mhyphen\mathsf{CMA}}}
\newcommand{\OTKEX}{\ensuremath{\mathsf{HAKE}}}
\newcommand{\indcpa}{\ensuremath{\mathsf{ind}\mhyphen\mathsf{cpa}}}

% COMMENTS
\newcommand{\ben}[1]{\textcolor{purple}{bd: #1}}
\newcommand{\kenny}[1]{\textcolor{red}{kgp: #1}}
\newcommand{\examplecomment}[1]{\textcolor{blue}{ex: #1}}

% WIREGUARD VARIABLES
\newcommand{\seed}{\ensuremath{C}}
\newcommand{\hash}{\ensuremath{H}}
\newcommand{\ID}[1]{\ensuremath{ID_{#1}}}
\newcommand{\wg}{\ensuremath{\mathsf{WG}}}
\newcommand{\mwg}{\ensuremath{\mathsf{mWG}}}
\newcommand{\wkey}{\ensuremath{\kappa}}
\newcommand{\PSK}{\ensuremath{psk}}
\newcommand{\now}{\ensuremath{now}}
\newcommand{\cookie}{\ensuremath{cookie}}
\newcommand{\tk}[1]{\ensuremath{tk_{#1}}}

% WIREGUARD MESSAGES AND FIELDS
\newcommand{\SendHello}{\ensuremath{\mathtt{InitiatorHello}}}  %% changed from send to initiator for consistency with WG paper
\newcommand{\sSendHello}{\ensuremath{\mathtt{InitHello}}}
\newcommand{\ssSendHello}{\ensuremath{\mathtt{SH}}}
\newcommand{\RespHello}{\ensuremath{\mathtt{ResponderHello}}}
\newcommand{\sRespHello}{\ensuremath{\mathtt{RespHello}}}
\newcommand{\ssRespHello}{\ensuremath{\mathtt{RH}}}
\newcommand{\lbl}[1]{\ensuremath{\mathtt{label}_{#1}}}
\newcommand{\type}{\ensuremath{\mathtt{type}}}
\newcommand{\etk}{\ensuremath{\mathtt{etk}}}
\newcommand{\epk}{\ensuremath{\mathtt{epk}}}
\newcommand{\ltk}{\ensuremath{\mathtt{ltk}}}
\newcommand{\sid}[1]{\ensuremath{\mathtt{sid}_{#1}}}
\newcommand{\tstamp}{\ensuremath{\mathtt{time}}}
\newcommand{\firstmac}{\ensuremath{\mathtt{mac1}}}
\newcommand{\secondmac}{\ensuremath{\mathtt{mac2}}}
\newcommand{\zero}{\ensuremath{\mathtt{zero}}}

%% CGKA VARIABLES
\newcommand{\propmsg}{\ensuremath{P}}
\newcommand{\welmsg}{\ensuremath{W}}
\newcommand{\commsg}{\ensuremath{C}}
\newcommand{\roster}{\ensuremath{R}}
\newcommand{\info}{\ensuremath{\mathit{info}}}
\newcommand{\op}{\ensuremath{\mathit{op}}}

%% CGKA ALGORITHMS
\newcommand{\CGKA}{\ensuremath{\mathsf{CGKA}}}
\newcommand{\CCreate}{\ensuremath{\mathsf{Create}}}
\newcommand{\Commit}{\ensuremath{\mathsf{Commit}}}
\newcommand{\Process}{\ensuremath{\mathsf{Process}}}
\newcommand{\Key}{\ensuremath{\mathsf{Key}}}
\newcommand{\CAdd}{\ensuremath{\mathsf{Add}}}
\newcommand{\CRemove}{\ensuremath{\mathsf{Remove}}}
\newcommand{\Update}{\ensuremath{\mathsf{Update}}}
\renewcommand{\Join}{\ensuremath{\mathsf{Join}}}

% Notation


% Math
\newcommand{\probnot}[1]{\overline{#1}}
\newcommand{\bitsnum}[2]{{\ll \hspace{-0.25em} \mathbf{#1} \hspace{-0.25em} \gg}_{#2}}
\newcommand{\bitspace}[1]{\ensuremath{\{0,1\}^{#1}}}
\renewcommand{\concat}{\ensuremath{\mathbin{\|}}}
\mathchardef\mhyphen="2D

\newcommand{\assign}{\leftarrow}
\newcommand{\evaluatesto}{\Rightarrow}

\newcommand{\pairwisedistinct}{\pcalgostyle{PairwiseDistinct}}
\newcommand{\collision}{\pcalgostyle{Coll}}
\newcommand{\nocollision}{\pcalgostyle{NoColl}}



% Secure Pairwise Channels: Signal & Olm
\newcommand{\SecureChannel}{\pcalgostyle{SC}}
\newcommand{\SecureChannelKGen}{\SecureChannel.\pcalgostyle{KGen}}
\newcommand{\SecureChannelIKE}{\SecureChannel.\pcalgostyle{IKE}}
\newcommand{\SecureChannelEnc}{\SecureChannel.\pcalgostyle{Enc}}
\newcommand{\SecureChannelDec}{\SecureChannel.\pcalgostyle{Dec}}

\newcommand{\Signal}{\pcalgostyle{Signal}}
\newcommand{\SignalKGen}{\Signal.\pcalgostyle{KGen}}
\newcommand{\SignalIKE}{\Signal.\pcalgostyle{IKE}}
\newcommand{\SignalEnc}{\Signal.\pcalgostyle{Enc}}
\newcommand{\SignalDec}{\Signal.\pcalgostyle{Dec}}

\newcommand{\Olm}{\pcalgostyle{Olm}}
\newcommand{\OlmKGen}{\Olm.\pcalgostyle{KGen}}
\newcommand{\OlmIKE}{\Olm.\pcalgostyle{IKE}}
\newcommand{\OlmEnc}{\Olm.\pcalgostyle{Enc}}
\newcommand{\OlmDec}{\Olm.\pcalgostyle{Dec}}
\newcommand{\OlmCmp}{\Olm.\pcalgostyle{Cmp}}
\newcommand{\OlmAlgorithmString}{\ensuremath{\mathtt{m.olm.v1.curve25519-aes-sha2}}}
\newcommand{\OlmState}[1][]{\ifthenelse{\equal{#1}{}}{\pi_{\pcvar{olm}}}{\pi_{\pcvar{olm},#1}}}
\newcommand{\OlmStates}[1][]{\ifthenelse{\equal{#1}{}}{\Pi_{\pcvar{olm}}}{\Pi_{\pcvar{olm},#1}}}

\newcommand{\OlmIdentitySK}[1][]{\ifthenelse{\equal{#1}{}}{isk}{isk_{#1}}}
\newcommand{\OlmIdentityPK}[1][]{\ifthenelse{\equal{#1}{}}{ipk}{ipk_{#1}}}
\newcommand{\OlmEphemSK}[1][]{\ifthenelse{\equal{#1}{}}{esk}{esk_{#1}}}
\newcommand{\OlmEphemPK}[1][]{\ifthenelse{\equal{#1}{}}{epk}{epk_{#1}}}


% Megolm

\newcommand{\Megolm}{\pcalgostyle{Megolm}}
\newcommand{\MegolmReg}{\Megolm.\pcalgostyle{Register}}
\newcommand{\MegolmInit}{\Megolm.\pcalgostyle{Init}}
\newcommand{\MegolmAddDevice}{\Megolm.\pcalgostyle{Add}}
\newcommand{\MegolmRemoveDevice}{\Megolm.\pcalgostyle{Remove}}
\newcommand{\MegolmEnc}{\Megolm.\pcalgostyle{Encrypt}}
\newcommand{\MegolmDec}{\Megolm.\pcalgostyle{Decrypt}}
\newcommand{\MegolmAdv}{\Megolm.\pcalgostyle{Advance}}
\newcommand{\MegolmAlgorithmString}{\ensuremath{\mathtt{m.megolm.v1.aes-sha2}}}
\newcommand{\MegolmSignature}{\ensuremath{\sigma_{\pcvar{mg}}}}
\newcommand{\MegolmVersion}{\ensuremath{\pcvar{ver}}}
\newcommand{\MegolmState}[1][]{\ifthenelse{\equal{#1}{}}{\pi_{\pcvar{mg}}}{\pi_{\pcvar{mg},#1}}}
\newcommand{\MegolmStates}[1][]{\ifthenelse{\equal{#1}{}}{\Pi_{\pcvar{mg}}}{\Pi_{\pcvar{mg},#1}}}

\newcommand{\MegolmRatchet}{\pcalgostyle{MegolmRatchet}}
\newcommand{\MegolmRatchetInit}{\MegolmRatchet.\pcalgostyle{Init}}
\newcommand{\MegolmRatchetNext}{\MegolmRatchet.\pcalgostyle{Next}}
\newcommand{\MegolmRatchetAdv}{\MegolmRatchet.\pcalgostyle{Advance}}

\newcommand{\ratchetkdf}{\pcalgostyle{RatchetKDF}}
\newcommand{\ratchetkdfinit}{\ratchetkdf.\pcalgostyle{Init}}
\newcommand{\ratchetkdfnext}{\ratchetkdf.\pcalgostyle{Next}}

\newcommand{\ratchetgamenext}{\pcalgostyle{Next}}
\newcommand{\ratchetgamecomp}{\pcalgostyle{Compromise}}
\newcommand{\ratchetgamecompromise}{\ratchetgamecomp}

\newcommand{\MegolmKeysConst}{\mathtt{``MEGOLM\_KEYS"}}

\newcommand{\hhc}[2]{(#1, #2)\mathsf{-hierarchical\ hash\ chain}}

\newcommand{\jsonencode}{\pcalgostyle{JSON.Encode}}
\newcommand{\jsondecode}{\pcalgostyle{JSON.Decode}}

\newcommand{\MegolmPK}[1][]{\ifthenelse{\equal{#1}{}}{gpk}{gpk_{#1}}}
\newcommand{\MegolmSK}[1][]{\ifthenelse{\equal{#1}{}}{gsk}{gsk_{#1}}}
\newcommand{\MegolmIS}{\ensuremath{\mathfrak{S}_{\MegolmPK[]}}}
\newcommand{\MegolmOS}{\ensuremath{\mathfrak{S}_{\MegolmSK[]}}}

% Cross Signing / Verification Framework

\newcommand{\CrossSign}{\pcalgostyle{CrossSign}}
\newcommand{\CrossSignInit}{\CrossSign.\pcalgostyle{Init}}
\newcommand{\CrossSignSignUser}{\CrossSign.\pcalgostyle{SignUser}}
\newcommand{\CrossSignSignDevice}{\CrossSign.\pcalgostyle{SignDevice}}
\newcommand{\CrossSignVerifyDevice}{\CrossSign.\pcalgostyle{VerifyDevice}}
\newcommand{\CrossSignKeyUsage}{\mathsf{usage}}
\newcommand{\CrossSignConstantMaster}{\mathtt{master}}
\newcommand{\CrossSignConstantSelfSign}{\mathtt{self\_signing}}
\newcommand{\CrossSignConstantUserSign}{\mathtt{user\_signing}}
\newcommand{\CrossSignState}[1][]{\ifthenelse{\equal{#1}{}}{\pi_{\pcvar{cs}}}{\pi_{\pcvar{cs},#1}}}
\newcommand{\CrossSignUserKeyPackage}[1]{u_{#1}}
\newcommand{\CrossSignDeviceRegistration}{\rho_{\pcvar{reg}}}
\newcommand{\CrossSignUserTrust}{\rho_{\pcvar{trust}}}
\newcommand{\MasterSK}[1][]{\ifthenelse{\equal{#1}{}}{msk}{msk_{#1}}}
\newcommand{\MasterPK}[1][]{\ifthenelse{\equal{#1}{}}{mpk}{mpk_{#1}}}
\newcommand{\UserSK}[1][]{\ifthenelse{\equal{#1}{}}{usk}{usk_{#1}}}
\newcommand{\UserPK}[1][]{\ifthenelse{\equal{#1}{}}{upk}{upk_{#1}}}
\newcommand{\SelfSK}[1][]{\ifthenelse{\equal{#1}{}}{ssk}{ssk_{#1}}}
\newcommand{\SelfPK}[1][]{\ifthenelse{\equal{#1}{}}{spk}{spk_{#1}}}

\newcommand{\CrossSignStateUnpack}
{(d, u, t, \MasterSK, \UserSK, \SelfSK) \assign \CrossSignState}
\newcommand{\CrossSignStatePack}
{\CrossSignState \assign (d, u, t, \MasterSK, \UserSK, \SelfSK)}


% SAS

\newcommand{\SAS}{\ensuremath{\pcalgostyle{SAS}}\xspace}
\newcommand{\SASCalculateMAC}{\ensuremath{\SAS.\pcalgostyle{CalcMAC}}\xspace}
\newcommand{\SASSendMAC}{\ensuremath{\SAS.\pcalgostyle{SendMAC}}\xspace}
\newcommand{\SASVerifyMAC}{\ensuremath{\SAS.\pcalgostyle{VerifyMAC}}\xspace}
\newcommand{\SASSignMAC}{\ensuremath{\SAS.\pcalgostyle{SignDevice}}\xspace}

\newcommand{\MsgTypeVerificationMAC}{%
	\ifmmode \mathtt{m.key.verification.mac}\xspace%
	\else \texttt{m.key.verification.mac}\xspace%
	\fi%
}


% Key Sharing

\newcommand{\KeyShare}{\pcalgostyle{KeyShare}}
\newcommand{\KeyShareRequest}{\KeyShare.\pcalgostyle{Request}}
\newcommand{\KeyShareShare}{\KeyShare.\pcalgostyle{Share}}
\newcommand{\KeyShareRecover}{\KeyShare.\pcalgostyle{Recover}}


% Secrets Module

\newcommand{\MsgTypeSecretsRequest}{%
	\ifmmode \mathtt{m.secret.requests}\xspace%
	\else \texttt{m.secret.requests}\xspace%
	\fi%
}

\newcommand{\MsgTypeSecretsSend}{%
	\ifmmode \mathtt{m.secret.send}\xspace%
	\else \texttt{m.secret.send}\xspace%
	\fi%
}


% Matrix Messaging

\newcommand{\Matrix}{\ensuremath{\pcalgostyle{Matrix}}}
\newcommand{\MatrixGen}{\ensuremath{\Matrix.\pcalgostyle{Gen}}}
\newcommand{\MatrixReg}{\ensuremath{\Matrix.\pcalgostyle{Reg}}}
\newcommand{\MatrixInit}{\ensuremath{\Matrix.\pcalgostyle{Init}}}
\newcommand{\MatrixRecv}{\ensuremath{\Matrix.\pcalgostyle{Recv}}}
\newcommand{\MatrixExec}{\ensuremath{\Matrix.\pcalgostyle{Exec}}}
\newcommand{\MatrixAdd}{\ensuremath{\Matrix.\pcalgostyle{Add}}}
\newcommand{\MatrixRemove}{\ensuremath{\Matrix.\pcalgostyle{Remove}}}
\newcommand{\MatrixEncrypt}{\ensuremath{\Matrix.\pcalgostyle{Encrypt}}}
\newcommand{\MatrixDecrypt}{\ensuremath{\Matrix.\pcalgostyle{Decrypt}}}
\newcommand{\MatrixKeyRequest}{\ensuremath{\Matrix.\pcalgostyle{KeyRequest}}}
\newcommand{\MatrixKeyShare}{\ensuremath{\Matrix.\pcalgostyle{KeyShare}}}
\newcommand{\MatrixKeyRecover}{\ensuremath{\Matrix.\pcalgostyle{KeyRecover}}}
\newcommand{\MatrixState}{\ensuremath{\pi_{\pcvar{mt}}}}

\newcommand{\DeviceKeyPackage}{m_{\pcvar{dev}}}  % A self-signed package for the device identity
\newcommand{\Algorithm}{\pcvar{alg}}
\newcommand{\DeviceMapping}[1][]{\ifthenelse{\equal{#1}{}}{\pcvar{DM}}{\pcvar{DM}_{#1}}}

\newcommand{\MsgTypeEncrypted}{%
	\ifmmode \mathtt{m.room.encrypted}\xspace%
	\else \texttt{m.room.encrypted}\xspace%
	\fi%
}
\newcommand{\MsgTypeMessage}{%
	\ifmmode \mathtt{m.room.message}\xspace%
	\else \texttt{m.room.message}\xspace%
	\fi%
}
\newcommand{\MsgTypeRoomKey}{%
	\ifmmode \mathtt{m.room\_key}\xspace%
	\else \texttt{m.room\_key}\xspace%
	\fi%
}
\newcommand{\MsgTypeRoomKeyRequest}{%
	\ifmmode \mathtt{m.room\_key\_request}\xspace%
	\else \texttt{m.room\_key\_request}\xspace%
	\fi%
}
\newcommand{\MsgTypeFwdRoomKey}{%
	\ifmmode \mathtt{m.forwarded\_room\_key}\xspace%
	\else \texttt{m.forwarded\_room\_key}\xspace%
	\fi%
}

\newcommand{\DeviceSK}[1][]{\ifthenelse{\equal{#1}{}}{dsk}{dsk_{#1}}}
\newcommand{\DevicePK}[1][]{\ifthenelse{\equal{#1}{}}{dpk}{dpk_{#1}}}

\newcommand{\MatrixStateUnpack}
{(U, D, G, \role, \DeviceMapping, \CrossSignState, \MegolmStates, \OlmStates, T) \assign \MatrixState}
\newcommand{\MatrixStatePack}
{\MatrixState \assign (U, D, G, \role, \DeviceMapping, \CrossSignState, \MegolmStates, \OlmStates, T)}

% Homeserver

\newcommand{\HS}{\pcalgostyle{HS}}
\newcommand{\HSGetDevicePK}{\HS.\pcalgostyle{GetDevicePK}}
\newcommand{\HSGetDeviceKeys}{\HS.\pcalgostyle{GetDeviceKeys}}
\newcommand{\HSGetCrossSigningMasterPK}{\HS.\pcalgostyle{GetCrossSigningMasterPK}}



% Ciphertext types
%
% Encrypted messages in Matrix can be wrapped in a few layers. Usually:
%   1. Actual message
%   2. (1) wrapped with event metadata like the event type (e.g. m.room_key), room_id etc.
%   3. Encryption of (2) by Olm or Megolm
%   4. Unauthenticated, plaintext wrapper of (3). This is the m.room.encrypted message.
%
% I had been using inconsistent notation to refer to these and it was all a bit confusing.
% Let's standardise it with the commands below:

\newcommand{\MsgPlaintext}{m}
\newcommand{\MsgCiphertext}{c}


% Crypto Primitives

\DeclareMathOperator{\hkdf}{\mathsf{HKDF}}
\DeclareMathOperator{\hmac}{\mathsf{HMAC}}
\DeclareMathOperator{\sha256}{\mathsf{SHA-256}}
\DeclareMathOperator{\hkdfsha256}{\mathsf{HKDF\mhyphen SHA\mhyphen 256}}
\DeclareMathOperator{\hmacsha256}{\mathsf{HMAC\mhyphen SHA\mhyphen 256}}
\DeclareMathOperator{\aescbc}{\mathsf{AES}\mhyphen\mathsf{CBC}}

\newcommand{\XDH}{\pcalgostyle{X25519}}
\newcommand{\XDHKGen}{\XDH.\kgen}
\newcommand{\XDHSklen}{{\XDH.\pcalgostyle{skl}}}
\newcommand{\XDHPklen}{{\XDH.\pcalgostyle{pkl}}}

\newcommand{\ed}{\pcalgostyle{Ed25519}}
\newcommand{\edkgen}{\ed.\kgen}
\newcommand{\edsign}{\ed.\pcalgostyle{Sign}}
\newcommand{\edverify}{\ed.\pcalgostyle{Verify}}
\newcommand{\edsklen}{{\ed.\pcalgostyle{skl}}}
\newcommand{\edpklen}{{\ed.\pcalgostyle{pkl}}}

\newcommand{\ds}{\pcalgostyle{DS}}
\newcommand{\dskgen}{{\ds.\kgen}}
\newcommand{\dssign}{{\ds.\pcalgostyle{Sign}}}
\newcommand{\dsverify}{\ds.\pcalgostyle{Verify}}
\newcommand{\dssklen}{{\ds.\pcalgostyle{skl}}}
\newcommand{\dspklen}{{\ds.\pcalgostyle{pkl}}}

\newcommand{\se}{\pcalgostyle{SE}}
\newcommand{\seenc}{{\se.\enc}}
\newcommand{\sedec}{{\se.\dec}}

\newcommand{\ff}{\pcalgostyle{F}}
\newcommand{\iv}{\pckeystyle{iv}}
\newcommand{\AD}{\mathit{AD}}
\newcommand{\pcvar}[1]{\mathsf{#1}}

\newcommand{\UGKE}{\pcalgostyle{UGKE}}
\newcommand{\PUGKE}{\pcalgostyle{PUGKE}}
\newcommand{\DOGM}{\ensuremath{\mathbf{DOGM}}}
\newcommand{\Reg}{\mathbf{Reg}}
\newcommand{\Add}{\mathbf{Add}}
\newcommand{\Remove}{\mathbf{Remove}}
\newcommand{\Encrypt}{\mathbf{Encrypt}}
\newcommand{\Decrypt}{\mathbf{Decrypt}}
\newcommand{\Gen}{\mathbf{Gen}}
\newcommand{\Exec}{\pcalgostyle{Exec}}
\newcommand{\Init}{\mathbf{Init}}
\newcommand{\Proc}{\pcalgostyle{Proc}}
\newcommand{\ProcAdd}{\pcalgostyle{ProcessAdd}}
\newcommand{\ProcRemove}{\pcalgostyle{ProcessRemove}}
\newcommand{\StateRecv}{\pcalgostyle{StateRecv}}
\newcommand{\StateShare}{\mathbf{StateShare}}
\newcommand{\StateReq}{\pcalgostyle{StateReq}}

%% PROTOCOL INTERFACES
\newcommand{\mem}{\pcalgostyle{mem}}
\newcommand{\rec}{\pcalgostyle{rec}}
\newcommand{\pau}{\pcalgostyle{pau}}


% ALGORITHMS
\renewcommand{\adversary}{\ensuremath{\mathcal{A}}}

%% SPACES
\newcommand{\pauspace}{\ensuremath{\mathcal{P}_{k}}}
\newcommand{\sauspace}{\ensuremath{\mathcal{S}_{k}}}
\newcommand{\psspace}{\ensuremath{\mathcal{PSS}}}
\newcommand{\sstate}{\ensuremath{\mathcal{ST}}}
\newcommand{\iid}{\ensuremath{\mathcal{IID}}}

\newcommand{\kidpace}{\ensuremath{\mathcal{K}_{id}}}
\newcommand{\gidspace}{\ensuremath{\mathcal{G}_{id}}}
\newcommand{\didspace}{\ensuremath{\mathcal{D}_{id}}}
\newcommand{\uidspace}{\ensuremath{\mathcal{U}_{id}}}

\newcommand{\uid}{\ensuremath{A}}
\newcommand{\did}{\ensuremath{i}}
\newcommand{\gid}{\ensuremath{G}}

\newcommand{\cmd}{\ensuremath{\mathcal{CMD}}}
\newcommand{\ctxt}{\ensuremath{\mathcal{C}}}
\newcommand{\keyspace}{\ensuremath{\mathcal{K}}}
\newcommand{\sidspace}{\ensuremath{\mathcal{SID}}}
\newcommand{\msgspace}{\ensuremath{\mathcal{M}}}

% EXPERIMENT CONSTANTS
\newcommand{\numComm}{\ensuremath{n_C}}
\newcommand{\numDevice}{\ensuremath{n_D}}
\newcommand{\numGroups}{\ensuremath{n_G}}
\newcommand{\numMsg}{\ensuremath{n_M}}
\newcommand{\send}{\ensuremath{\styleConstants{send}}}
\newcommand{\recv}{\ensuremath{\styleConstants{recv}}}
%\newcommand{\numX}{\ensuremath{n_X}}

% EXPERIMENT FLAGS
\newcommand{\DKflag}[2]{\ensuremath{\mathsf{DKflag}_{#1}^{#2}}}
\newcommand{\GSflag}[2]{\ensuremath{\mathsf{GSflag}_{#1}^{#2}}}
\newcommand{\USflag}[1]{\ensuremath{\mathtt{UsS}_{#1}}}
\newcommand{\DSflag}[1]{\ensuremath{\mathtt{DeS}_{#1}}}
\newcommand{\SSflag}[1]{\ensuremath{\mathtt{SeS}_{#1}}}

% SESSIONS AND PER-SESSION VARIABLES
\renewcommand{\state}{\ensuremath{st}}
\newcommand{\clean}{\ensuremath{clean}}

% SECURITY GAME QUERIES
\newcommand{\CorruptUser}{\ensuremath{\mathsf{CorruptUser}}}
\newcommand{\CorruptDevice}{\ensuremath{\mathsf{CorruptDevice}}}
\newcommand{\Compromise}{\ensuremath{\mathsf{Compromise}}}
\newcommand{\AddMember}{\ensuremath{\mathsf{AddMember}}}
\newcommand{\RemoveMember}{\ensuremath{\mathsf{RemoveMember}}}
\newcommand{\Chall}{\mathsf{Challenge}}



% SECURITY GAME NOTIONS
\newcommand{\PFSUGKE}{\ensuremath{\mathsf{PFS}\mhyphen \mathsf{UGKE}}}
\newcommand{\KIND}{\ensuremath{\mathsf{KIND}}}


% Crypto Games

\newcommand{\game}[2]{\pcalgostyle{Game}^{\mathcal{#1}}_{\pcalgostyle{#2}}}


% Security Definitions

\newcommand{\rkdfsecure}[3]{(#1, #2, #3)\textsf{-secure ratcheted key derivation function}}


% Actors/variable scoping

\definecolor{scopeprivate}{RGB}{255,99,71}
\definecolor{scopeinsider}{RGB}{0,205,00}
\definecolor{scopeoutsider}{RGB}{58,95,255}

\newcommand{\scopeprivate}[1]{\textcolor{scopeprivate}{#1}}
\newcommand{\scopeinsider}[1]{\textcolor{scopeinsider}{#1}}
\newcommand{\scopeoutsider}[1]{\textcolor{scopeoutsider}{#1}}

\newcommand{\sessionout}{S^{\mathsf{OUT}}}
\newcommand{\sessionin}{S^{\mathsf{IN}}}

% Keys
\newcommand{\fingerprintkey}{\pckeystyle{fk}}
\newcommand{\olmkeys}{\pckeystyle{ok}}


% Pseudocode
\newcommand{\pcbreak}{\highlightkeyword{break}}


==> figure-macros.tex <==
% FIGURE COMMANDS
\definecolor{mBlue}{HTML}{22a1dc}
\definecolor{sBlue}{HTML}{009FE3}
\definecolor{sYellow}{HTML}{FFED00}
\definecolor{sRed}{HTML}{E30613}
\definecolor{sGreen}{HTML}{009640}
\definecolor{sPurple}{HTML}{440099}
\definecolor{mGreen}{HTML}{86cd30}
\definecolor{darkgreen}{HTML}{006400}
\definecolor{mLightBrown}{HTML}{e68a00}
\definecolor{lightred}{HTML}{FF9999}


%% MATH MODE COLOR BOXES
\newcommand{\highlight}[2][yellow]{\mathchoice%
	{\colorbox{#1}{$\displaystyle#2$}}%
	{\colorbox{#1}{$\textstyle#2$}}%
	{\colorbox{#1}{$\scriptstyle#2$}}%
	{\colorbox{#1}{$\scriptscriptstyle#2$}}}%

% ClientAction and ServerAction
% Print a command executed by the client/server
% 1st argument: the text
\newcommand{\ClientAction}[1]{
	\node[right] at (\InitX, \Y) {#1};
}
\newcommand{\ServerAction}[1]{
	\node[left] at (\RespX, \Y) {#1};
}
\newcommand{\SharedAction}[1]{
	\node at ($1/2*(\InitX, \Y)+1/2*(\RespX, \Y)$) {#1};
}
\newcommand{\AdversaryAction}[1]{
	\node at ($1/2*(\InitX, \Y)+1/2*(\RespX, \Y)$) {#1};
}

% ClientToServer and ServerToClient
% Draws a message flow from client-to-server or server-to-client, with text above and below
% 1st argument (optional): line type, default ->
% 2nd argument: text above
% 3rd argument: text below
% Example: \ClientToServer{$Y$}{}
% Example: \ClientToServer[<->,double]{$Y$}{over an encrypted channel}
\newcommand{\ClientToServer}[3][->]{
	\NextLine[0.5]
	\draw[#1] (\ArrowLeft,\Y) -- node[above] {#2} node[below] {#3} (\ArrowRight,\Y) ;
	\NextLine[0.5]
}
\newcommand{\ServerToClient}[3][->]{
	\NextLine[0.5]
	\draw[#1] (\ArrowRight,\Y) -- node[above] {#2} node[below] {#3} (\ArrowLeft,\Y) ;
	\NextLine[0.5]
}
\newcommand{\ClientToAdversary}[3][->]{
	\NextLine[0.5]
	\draw[#1] (\ArrowLeft,\Y) -- node[above] {#2} node[below] {#3} (\ArrowCenter,\Y) ;
	\NextLine[0.5]
}
\newcommand{\ServerToAdversary}[3][->]{
	\NextLine[0.5]
	\draw[#1] (\ArrowRight,\Y) -- node[above] {#2} node[below] {#3} (\ArrowCenter,\Y) ;
	\NextLine[0.5]
}
\newcommand{\AdversaryQToClient}[3][->]{
	\NextLine[0.5]
	\draw[#1] (\ArrowCenter,\Y) -- node[above] {\textcolor{red}{#2}} node[below] {#3} (\ArrowLeft,\Y) ;
	\NextLine[0.5]
}
\newcommand{\AdversaryQToServer}[3][->]{
	\NextLine[0.5]
	\draw[#1] (\ArrowCenter,\Y) -- node[above] {\textcolor{red}{#2}} node[below] {#3} (\ArrowRight,\Y) ;
	\NextLine[0.5]
}
\newcommand{\AdversaryToClient}[3][->]{
	\NextLine[0.5]
	\draw[#1] (\ArrowCenter,\Y) -- node[above] {#2} node[below] {#3} (\ArrowLeft,\Y) ;
	\NextLine[0.5]
}
\newcommand{\AdversaryToServer}[3][->]{
	\NextLine[0.5]
	\draw[#1] (\ArrowCenter,\Y) -- node[above] {#2} node[below] {#3} (\ArrowRight,\Y) ;
	\NextLine[0.5]
}
\newcommand{\Encryption}[3][<->]{
	\NextLine[0.5]
	\draw[#1] (\ArrowRight,\Y) -- node[above] {#2} node[below] {#3} (\ArrowLeft,\Y) ;
	\NextLine[0.5]
}
% NextLine
% 1st argument (optional): amount of spacing to increment by, default 1.0
% Example: \NextLine
% Example: \NextLine[1.5]
\newcommand{\NextLine}[1][1.0]{
	\pgfmathparse{\Y+#1}
	\edef\Y{\pgfmathresult}
}
%
% stage separator line
%
\newcommand{\StageSeparator}[2][1.0]{
	\draw[very thick,dotted,blue] (\InitX,\Y+0.5) node[above=-0.1cm,anchor=north west] {\bf #2} -- (\RespX,\Y+0.5);
}
\newcommand{\Separator}[2][1.0]{
	\draw[very thick,dotted,blue] (\InitX,\Y+0.5) node[above=-0.1cm,anchor=north west] {\bf #2} -- (\RespX,\Y+0.5);
}
\newcommand{\StageRight}[1]{
	\node[above=-0.1cm,anchor=north east,StageSeparatorColor] at
	(\RespX,\Y+0.5) {\bf #1};
}

% TIKZ PICTURES

\tikzset{cloud/.pic={
		\node[cloud, cloud puffs=10.8,cloud puff arc=110, aspect=4, draw, text width=2cm
		] () at (0,0) {\tikzpictext};
	}}

\tikzset{database/.style={
		cylinder,
		aspect=1,
		draw,
		thick,
		fill,
		shape border rotate=90,
		minimum height=1.5cm,
		left color=sGreen!30,
		right color=sGreen!30,
		middle color=sGreen!30,
		minimum width=2cm,
		path picture={
			\draw[black, thick] let \p1=($(path picture bounding box.north east)-(path picture bounding
			box.south west)$) in 
			foreach \XX in {1,2,3}  {([yshift=-\XX*\y1/4]path picture bounding box.north west) 
				arc(180:360:\x1/2 and 0.25*\x1/2)};
		}}}

\makeatletter
\tikzset{
	monodatabase/.style={
		path picture={
			\draw (0, 1.5*\database@segmentheight) circle [x radius=\database@radius,y radius=\database@aspectratio*\database@radius];
			\draw (-\database@radius, 0.5*\database@segmentheight) arc [start angle=180,end angle=360,x radius=\database@radius, y radius=\database@aspectratio*\database@radius];
			\draw (-\database@radius,-0.5*\database@segmentheight) arc [start angle=180,end angle=360,x radius=\database@radius, y radius=\database@aspectratio*\database@radius];
			\draw (-\database@radius,1.5*\database@segmentheight) -- ++(0,-3*\database@segmentheight) arc [start angle=180,end angle=360,x radius=\database@radius, y radius=\database@aspectratio*\database@radius] -- ++(0,3*\database@segmentheight);
		},
		minimum width=2*\database@radius + \pgflinewidth,
		minimum height=3*\database@segmentheight + 2*\database@aspectratio*\database@radius + \pgflinewidth,
	},
	database segment height/.store in=\database@segmentheight,
	database radius/.store in=\database@radius,
	database aspect ratio/.store in=\database@aspectratio,
	database segment height=0.1cm,
	database radius=0.25cm,
	database aspect ratio=0.35,
}
\makeatother

\tikzset{XOR/.style={draw,circle,append after command={
			[shorten >=\pgflinewidth, shorten <=\pgflinewidth,]
			(\tikzlastnode.north) edge (\tikzlastnode.south)
			(\tikzlastnode.east) edge (\tikzlastnode.west)
		}
	}
}

\newcommand{\boundellipse}[3]% center, xdim, ydim
{(#1) ellipse (#2 and #3)
}
